MiDAS: Multi-integrated Domain Adaptive Supervision for Fake News Detection

COVID-19 related misinformation and fake news, coined an 'infodemic', has dramatically increased over the past few years. This misinformation exhibits concept drift, where the distribution of fake news changes over time, reducing effectiveness of previously trained models for fake news detection. Given a set of fake news models trained on multiple domains, we propose an adaptive decision module to select the best-fit model for a new sample. We propose MiDAS, a multi-domain adaptative approach for fake news detection that ranks relevancy of existing models to new samples. MiDAS contains 2 components: a doman-invariant encoder, and an adaptive model selector. MiDAS integrates multiple pre-trained and fine-tuned models with their training data to create a domain-invariant representation. Then, MiDAS uses local Lipschitz smoothness of the invariant embedding space to estimate each model's relevance to a new sample. Higher ranked models provide predictions, and lower ranked models abstain. We evaluate MiDAS on generalization to drifted data with 9 fake news datasets, each obtained from different domains and modalities. MiDAS achieves new state-of-the-art performance on multi-domain adaptation for out-of-distribution fake news classification.

==> Makefile <==
# Makefile for LaTeX files

PACKAGE=acmart

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
PANDOC = pandoc

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS :=
#PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

.PHONY	: all show clean ps pdf showps text stylecheck spellcheck

view:
	acroread $(PDF)

osx:
	open $(PDF)

text: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

doc: *.tex
	$(PANDOC) --wrap=none -s $< -o $@

combined:
	pdfunite response.pdf logging.pdf combined.pdf

# Check style:
stylecheck:
	printf "weasel words: "
	sh ./scripts/weasel *.tex
	printf "\npassive voice: "
	sh ./scripts/passive *.tex
	printf "\nduplicates: "
	perl ./scripts/dups *.tex
	printf "\ndone\n"

# Check spelling with aspell
spellcheck:
	find . -name "*.tex" -exec aspell --lang=en --mode=tex --dont-suggest --personal=./.aspell.en.pws check "{}" \;

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)


docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.bak

distclean: docclean
	$(RM)  *.pdf 

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)

bclean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)


zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*' -x 'figs/*'
